Semi-parametric TEnsor Factor Analysis by Iteratively Projected Singular Value Decomposition

This paper introduces a general framework of Semi-parametric TEnsor Factor Analysis (STEFA) that focuses on the methodology and theory of low-rank tensor decomposition with auxiliary covariates. Semi-parametric TEnsor Factor Analysis models extend tensor factor models by incorporating auxiliary covariates in the loading matrices. We propose an algorithm of iteratively projected singular value decomposition (IP-SVD) for the semi-parametric estimation. It iteratively projects tensor data onto the linear space spanned by the basis functions of covariates and applies singular value decomposition on matricized tensors over each mode. We establish the convergence rates of the loading matrices and the core tensor factor. The theoretical results only require a sub-exponential noise distribution, which is weaker than the assumption of sub-Gaussian tail of noise in the literature. Compared with the Tucker decomposition, IP-SVD yields more accurate estimators with a faster convergence rate. Besides estimation, we propose several prediction methods with new covariates based on the STEFA model. On both synthetic and real tensor data, we demonstrate the efficacy of the STEFA model and the IP-SVD algorithm on both the estimation and prediction tasks.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
	if ( $root_filename ne $_[0] )  {
		my ($base_name, $path) = fileparse( $_[0] );
		pushd $path;
		my $return = system "latexmk",
		@sub_doc_options,
		"-aux-directory=$sub_doc_output",
		"-output-directory=$sub_doc_output",
		$base_name;
		if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
			# In this case, .aux file generated by pdflatex isn't in same
			# directory as the .tex file.
			# Therefore:
			# 1. Actual generated aux file must be listed as produced by this
			#    rule, so that latexmk deals with dependencies correctly.
			#    (Problem to overcome: If $sub_dir_output is same as $aux_dir
			#    for the main document, xr may read the .aux file in the
			#    aux_dir rather than the one the cus dep is assumed by latexmk
			#    to produce, which is in the same directory as the .tex source
			#    file for this custom dependency.)
			#    Use not-yet-documented latexmk subroutine rdb_add_generated
			#    to do this:
			# 2. A copy of the .aux file must be in same directory as .tex file
			#    to satisfy latexmk's definition of a custom dependency.
			rdb_add_generated( "$sub_doc_output/$base_name.aux" );
			copy "$sub_doc_output/$base_name.aux", ".";
		}
		popd;
		return $return;
	}
}

==> macros/algorithm.tex <==


% \usepackage{algorithm,algorithmicx,algpseudocode}
% http://shantoroy.com/latex/how-to-write-algorithm-in-latex/
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}} % require \usepackage{xcolor}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

==> macros/box-theorems.tex <==
% more info here
% https://texblog.org/2015/09/30/fancy-boxes-for-theorem-lemma-and-proof-with-mdframed/

\usepackage[framemethod=TikZ]{mdframed} % box environment & flexible box designs

% or
\usepackage{fancybox}

==> macros/code.tex <==

%%
%%  code listing macros
%%

%% refs: https://www.overleaf.com/learn/latex/Code_listing

\usepackage{listings}             % Include the listings-package
\lstset{basicstyle=\ttfamily,
	showstringspaces=false,
	commentstyle=\color{red},
	keywordstyle=\color{blue}
}

==> macros/self-defined.tex <==
% Copy right @ 2019
% All right reserved by Elynn Y. Chen.
% This file defines short-hands for math formulas.
% It started with  Prof. Jianqing Fan's macro definition.
% Later it incorporated some of my own macro definition.
%
%
% Other references:
% -- math guide: http://mirrors.rit.edu/CTAN/info/short-math-guide/short-math-guide.pdf
% -- bold math symbol: https://tex.stackexchange.com/questions/595/how-can-i-get-bold-math-symbols
%
%

\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}

%--------------------------------
%
%  Boldfaces in Letters
%
% \newcommand{\bfm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\bfm}[1]{\ensuremath{\boldsymbol{#1}}} % bm

\def\bzero{\bfm 0}
\def\bone{\bfm 1}
\def\bbone{\mathbbm{1}} % package bm

\def\ba{\bfm a}   \def\bA{\bfm A}  \def\AA{\mathbb{A}}
\def\bb{\bfm b}   \def\bB{\bfm B}  \def\BB{\mathbb{B}}
\def\bc{\bfm c}   \def\bC{\bfm C}  \def\CC{\mathbb{C}}
\def\bd{\bfm d}   \def\bD{\bfm D}  \def\DD{\mathbb{D}}
\def\be{\bfm e}   \def\bE{\bfm E}  \def\EE{\mathbb{E}}
\def\bff{\bfm f}  \def\bF{\bfm F}  \def\FF{\mathbb{F}}
\def\bg{\bfm g}   \def\bG{\bfm G}  \def\GG{\mathbb{G}}
\def\bh{\bfm h}   \def\bH{\bfm H}  \def\HH{\mathbb{H}}
\def\bi{\bfm i}   \def\bI{\bfm I}  \def\II{\mathbb{I}}
\def\bj{\bfm j}   \def\bJ{\bfm J}  \def\JJ{\mathbb{J}}
\def\bk{\bfm k}   \def\bK{\bfm K}  \def\KK{\mathbb{K}}
\def\bl{\bfm l}   \def\bL{\bfm L}  \def\LL{\mathbb{L}}
\def\bm{\bfm m}   \def\bM{\bfm M}  \def\MM{\mathbb{M}}
\def\bn{\bfm n}   \def\bN{\bfm N}  \def\NN{\mathbb{N}}
\def\bo{\bfm o}   \def\bO{\bfm O}  \def\OO{\mathbb{O}}
\def\bp{\bfm p}   \def\bP{\bfm P}  \def\PP{\mathbb{P}}
\def\bq{\bfm q}   \def\bQ{\bfm Q}  \def\QQ{\mathbb{Q}}
\def\br{\bfm r}   \def\bR{\bfm R}  \def\RR{\mathbb{R}}
\def\bs{\bfm s}   \def\bS{\bfm S}  \def\SS{\mathbb{S}}
\def\bt{\bfm t}   \def\bT{\bfm T}  \def\TT{\mathbb{T}}
\def\bu{\bfm u}   \def\bU{\bfm U}  \def\UU{\mathbb{U}}
\def\bv{\bfm v}   \def\bV{\bfm V}  \def\VV{\mathbb{V}}
\def\bw{\bfm w}   \def\bW{\bfm W}  \def\WW{\mathbb{W}}
\def\bx{\bfm x}   \def\bX{\bfm X}  \def\XX{\mathbb{X}}
\def\by{\bfm y}   \def\bY{\bfm Y}  \def\YY{\mathbb{Y}}
\def\bz{\bfm z}   \def\bZ{\bfm Z}  \def\ZZ{\mathbb{Z}}

\def\calA{{\cal  A}} \def\cA{{\cal  A}}
\def\calB{{\cal  B}} \def\cB{{\cal  B}}
\def\calC{{\cal  C}} \def\cC{{\cal  C}}
\def\calD{{\cal  D}} \def\cD{{\cal  D}}
\def\calE{{\cal  E}} \def\cE{{\cal  E}}
\def\calF{{\cal  F}} \def\cF{{\cal  F}}
\def\calG{{\cal  G}} \def\cG{{\cal  G}}
\def\calH{{\cal  H}} \def\cH{{\cal  H}}
\def\calI{{\cal  I}} \def\cI{{\cal  I}}
\def\calJ{{\cal  J}} \def\cJ{{\cal  J}}
\def\calK{{\cal  K}} \def\cK{{\cal  K}}
\def\calL{{\cal  L}} \def\cL{{\cal  L}}
\def\calM{{\cal  M}} \def\cM{{\cal  M}}
\def\calN{{\cal  N}} \def\cN{{\cal  N}}
\def\calO{{\cal  O}} \def\cO{{\cal  O}}
\def\calP{{\cal  P}} \def\cP{{\cal  P}}
\def\calQ{{\cal  Q}} \def\cQ{{\cal  Q}}
\def\calR{{\cal  R}} \def\cR{{\cal  R}}
\def\calS{{\cal  S}} \def\cS{{\cal  S}}
\def\calT{{\cal  T}} \def\cT{{\cal  T}}
\def\calU{{\cal  U}} \def\cU{{\cal  U}}
\def\calV{{\cal  V}} \def\cV{{\cal  V}}
\def\calW{{\cal  W}} \def\cW{{\cal  W}}
\def\calX{{\cal  X}} \def\cX{{\cal  X}}
\def\calY{{\cal  Y}} \def\cY{{\cal  Y}}
\def\calZ{{\cal  Z}} \def\cZ{{\cal  Z}}

\def\calh{{\cal h}}

%--------------------------------
%
%  Boldfaces in Greek
%
\newcommand{\bfsym}[1]{\ensuremath{\boldsymbol{#1}}}

 \def\balpha{\bfsym \alpha}
 \def\bbeta{\bfsym \beta}
 \def\bgamma{\bfsym \gamma}             \def\bGamma{\bfsym \Gamma}
 \def\bdelta{\bfsym {\delta}}           \def\bDelta {\bfsym {\Delta}}
 \def\bfeta{\bfsym {\eta}}              \def\bfEta {\bfsym {\Eta}}
 \def\bmu{\bfsym {\mu}}                 \def\bMu {\bfsym {\Mu}}
 \def\bnu{\bfsym {\nu}}
 \def\btheta{\bfsym {\theta}}           \def\bTheta {\bfsym {\Theta}}
 \def\beps{\bfsym \varepsilon}          \def\bEps{\bfsym{\mathcal E}}
 \def\bepsilon{\bfsym \varepsilon}
 \def\bsigma{\bfsym \sigma}             \def\bSigma{\bfsym \Sigma}
  \def\bsig{\bfsym \sigma}             \def\bSig{\bfsym \Sigma}
 \def\blambda {\bfsym {\lambda}}        \def\bLambda {\bfsym {\Lambda}}
 \def\bomega {\bfsym {\omega}}          \def\bOmega {\bfsym {\Omega}}
 \def\brho   {\bfsym {\rho}}
 \def\btau{\bfsym {\tau}}
 \def\bxi{\bfsym {\xi}}          \def\bXi{\bfsym {\Xi}}
 \def\bzeta{\bfsym {\zeta}}
 \def\bpi{\bfsym {\pi}}          \def\bPi{\bfsym {\Pi}}
\def\bphi{\bfsym {\phi}}          \def\bPhi{\bfsym {\Phi}}
\def\bpsi{\bfsym {\psi}}          \def\bPsi{\bfsym {\Psi}}
\def\bchi{\bfsym {\chi}}          \def\bChi{\bfsym {\Chi}}
\def\bupsi{\bfsym {\upsilon}}          \def\bUpsi{\bfsym {\Upsilon}}

 %--------------------------------
 %
 %  Hat (boldface) in Greek
 %
  \def\halpha{\hat{\alpha}}              \def\hbalpha{\hat{\bfsym \alpha}}
  \def\hbeta{\hat{\beta}}                \def\hbbeta{\hat{\bfsym \beta}}
  \def\hgamma{\hat{\gamma}}              \def\hgamma{\hat{\bfsym \gamma}}
  \def\hGamma{\hat{ \Gamma}}             \def\hbGamma{\hat{\bfsym \Gamma}}
  \def\hdelta{\hat{\delta}}              \def\hbdelta{\hat{\bfsym {\delta}}}
  \def\hDelta {\hat{\Delta}}             \def\hbDelta{\hat{\bfsym {\Delta}}}
  \def\heta{\hat {\eta}}                 \def\hbfeta {\hat{\bfsym {\eta}}}
  \def\hmu{\hat{\mu}}                    \def\hbmu {\hat{\bfsym {\mu}}}
  \def\hnu{\hat{\nu}}                    \def\hbnu {\hat{\bfsym {\nu}}}
  \def\htheta{\hat {\theta}}             \def\hbtheta {\hat{\bfsym {\theta}}}
  \def\hTheta{\hat {\Theta}}             \def\hbTheta {\hat{\bfsym {\Theta}}}
  \def\hbeps{\hat{\bfsym \varepsilon}}   \def\hbepsilon{\hat{\bfsym \varepsilon}}
  \def\hsigma{\hat{\sigma}}              \def\hbsigma{\hat{\bfsym \sigma}}
  \def\hSigma{\hat{\Sigma}}              \def\hbSigma{\hat{\bfsym \Sigma}}
  \def\hlambda{\hat{\lambda}}            \def\hblambda{\hat{\bfsym \lambda}}
  \def\hLambda{\hat{\Lambda}}            \def\hbLambda{\hat{\bfsym \Lambda}}
  \def\homega {\hat {\omega}}            \def\hbomega {\hat{\bfsym {\omega}}}
  \def\hOmega {\hat {\omega}}            \def\hbOmega {\hat{\bfsym {\Omega}}}
  \def\hrho   {\hat {\rho}}              \def\hbrho {\hat{\bfsym {\rho}}}
  \def\htau   {\hat {\tau}}              \def\hbtau {\hat{\bfsym {\tau}}}
  \def\hxi{\hat{\xi}}                    \def\hbxi{\hat{\bfsym {\xi}}}
  \def\hzeta{\hat{\zeta}}                \def\hbzeta{\hat{\bfsym {\bzeta}}}


 %--------------------------------
 %
 %  Operator
 %
\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\providecommand{\angles}[1]{\left\langle #1 \right\rangle}
\providecommand{\paran}[1]{\left( #1 \right)}
\providecommand{\brackets}[1]{\left[ #1 \right]}
\providecommand{\braces}[1]{\left\{ #1 \right\}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\providecommand{\convprob}{\stackrel{\calP}{\longrightarrow}}
\providecommand{\convdist}{\stackrel{\calD}{\longrightarrow}}
\providecommand{\defeq}{\triangleq}
% \providecommand{\defeq}{\dot{=}}

\usepackage{mathtools}
% K-L divergence
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1 \; \delimsize\| \; #2%
}
\newcommand{\infdiv}{\calD \infdivx}
\newcommand{\kldiv}{\calD_{KL} \infdivx}

%--------------------------------
%
% Regular font in math equation
%

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\corr}{corr}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Dev}{Dev}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\E}{E}
\newcommand{\E}[1]{{\mathbb{E}} \left[ #1 \right]}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\RSS}{RSS}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\SE}{SE}
\DeclareMathOperator{\Prob}{Pr}
%\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
%\DeclareMathOperator{\vect}{vec}
\newcommand{\vect}[1]{{\textsc{vec}} \left( #1 \right)}
\newcommand{\mat}[1]{{\textsc{mat}} \left( #1 \right)}


%--------------------------------
%
%  Thms, Props, Assumps, Remarks, et al
%

%\newtheorem{definition}{Definition}[section]
%\newtheorem{assumption}[definition]{Assumption}
%\newtheorem{lemma}[definition]{Lemma}
%\newtheorem{proposition}[definition]{Proposition}
%\newtheorem{theorem}[definition]{Theorem}
%\newtheorem{corollary}[definition]{Corollary}
%\newtheorem{exercise}[definition]{Exercise}
%\newtheorem{example}[definition]{Example}
%
%\newenvironment{solution}{\paragraph{Solution:}}{\hfill$\square$}
%
%\renewcommand*{\theassumption}{\Alph{assumption}}

\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}

%\def\remark{{\noindent\underbar{\bf Remark}\quad}}
\newtheorem{remark}{Remark}

%--------------------------------
%
%  Bachmann-Landau or asymptotic notations
%
% determiniastic convergence
\newcommand{\bigO}[1]{ \mathcal{O} \left( #1 \right) }
\newcommand{\bigOmega}[1]{ \Omega \left( #1 \right) }
\newcommand{\bigTheta}[1]{ \Theta \left( #1 \right) }
\newcommand{\smlo}[1]{{\rm o} \left( #1 \right) }
\newcommand{\smlomega}[1]{{\omega} \left( #1 \right) }

% converge in probability
\newcommand{\Op}[1]{{\mathcal{O}_p} \left( #1 \right) }
\newcommand{\op}[1]{{\rm o_p} \left( #1 \right) }

%--------------------------------
%
%  Markers
%
% need \usepackage[table,xcdraw,dvipsnames]{xcolor}   % for \textcolor

% colorful text emphasizer
\providecommand{\textem}[1]{\textit{\textcolor{Cerulean}{#1}}}

% comments
\definecolor{royalpurple}{rgb}{0.47, 0.32, 0.66}
\providecommand{\elynn}[1]{\textcolor{RubineRed}{\bf [Elynn: #1]}}
\providecommand{\attn}[1]{\textcolor{red}{\bf (#1)}}
\providecommand{\xuening}[1]{\textcolor{blue}{\bf [Xuening: #1]}}

 %--------------------------------
%
%  Semi-parametric specials
%

\newcommand{\jbracket}[1]{ J_{[]}\braces{#1} }
\newcommand{\nbracket}[1]{ N_{[]}\braces{#1} }

 %--------------------------------
 %
 %  Shorthands
 %

\def\eps{\varepsilon}
\def\lam {\lambda}
\def\blam {\blambda}
\def\bLam {\bLambda}
\def\bdiag{{\rm bdiag}}

\def\vec{\mbox{vec}}
\def\wh{\widehat}
\def\blue{\color{blue}}
\def\red{\color{red}}

% May add more in future.

\newenvironment{question}{ \color{teal} \textbf{To settle:}  }{\hfill$\clubsuit$}


==> tex-pool.tex <==


%\begin{enumerate}[label=\textbf{Step \arabic*.}, leftmargin=*]
%    \item \textit{(Projected spectral initialization)}
%    By sieve approximation, the column space of each loading $\bG_m$ is mainly a subspace of the basis projection $\bP_m$.
%    Therefore, a preliminary estimator for $\bG_m$, $m\in[3]$, is attainable via sieve projection, matricization and singular value decomposition (SVD) in equation \eqref{eqn:initialization}. 
%    \begin{equation*}
    %    \begin{aligned}
        %    \tilde\calY &= \calY \times_1 \bP_1 \times_2 \bP_2 \times_3 \bP_3 \quad {\rm and}\quad
        %    \tilde \bG_m^{(0)} &= \sqrt{I_m}\cdot{\rm SVD}_{R_m}(\calM_m(\tilde\calY)),
        %    \end{aligned}
    %    \end{equation*}
%    where $\text{\rm SVD}_{R_m}(\cdot)$ returns the first $R_m$ left singular vectors of a matrix.
%    This step, in spirit, is similar to the projected PCA in \citep{fan2016projected}.
%    $\tilde \bG_m^{(0)}$ acts as a good starting point, but is {\em sub-optimal} in general.

%    \item \textit{(Projected power iteration)}
%    We apply power iterations to refine the initializations.

%    Therefore, for $t=1,\cdots,t_{\max}$, we compute
%    \begin{equation*}
    %    \begin{split}
        %    \tilde\bG_1^{(t)} &= \sqrt{I_1}\cdot{\rm SVD}_{R_1}\paran{ \bP_1\calM_1\paran{\calY \times_2 \tilde\bG_2^{(t-1)\top} \times_3 \tilde\bG_3^{(t-1)\top}}},\\
        %    \tilde \bG_2^{(t)} &=\sqrt{I_2}\cdot {\rm SVD}_{R_2}\paran{\bP_2\calM_2\paran{\calY\times_1 \tilde\bG_1^{(t)\top} \times_3 \tilde\bG_3^{(t-1)\top}} },\\
        %    \tilde \bG_3^{(t)} &= \sqrt{I_3}\cdot{\rm SVD}_{R_3}\paran{\bP_3\calM_3\paran{\calY\times_1 \tilde \bG_1^{(t)\top} \times_2 \tilde \bG_2^{(t)\top}}}.
        %    \end{split}
    %    \end{equation*}
%    This projected power iteration algorithm is a modification of the classical HOOI algorithm \citep{de2000best}.
%    The additional projection $\bP_m$ restricts the solution to be a linear function of sieve basis functions.
%    Empirically, the projected version of HOOI in this step converges very fast within a few iterations.

%    \item \textit{(Projection estimate for tensor factor)}
%    After obtaining the final estimates $\tilde \bG_m=\tilde \bG_m^{(t_{\max})}$ from Step~2, it is natural to estimate $\calF$ via least squares which amounts to the projection in equation \eqref{eqn:proj-F}. 
%    $\tilde \calF = (I_1I_2I_3)^{-1}\cdot \calY \times_1 \tilde \bG_1^\top \times_2 \tilde \bG_2^\top \times_3 \tilde \bG_3^\top$.

%    \item \textit{(Orthogonal calibration)} 
%    \begin{equation*}
    %    \hat\calF=\tilde\calF\times_1\hat \bO_1^{\top}\times_2 \bO_2^{\top} \times_3 \hat \bO_3^{\top}\quad {\rm and}\quad \hat\bG_m=\tilde\bG_m\hat\bO_m,\ m\in [3].
    %    \end{equation*}
%\end{enumerate}
